Semantic Tracklets: An Object-Centric Representation for Visual Multi-Agent Reinforcement Learning

Solving complex real-world tasks, e.g., autonomous fleet control, often involves a coordinated team of multiple agents which learn strategies from visual inputs via reinforcement learning. Many existing multi-agent reinforcement learning (MARL) algorithms however don't scale to environments where agents operate on visual inputs. To address this issue, algorithmically, recent works have focused on non-stationarity and exploration. In contrast, we study whether scalability can also be achieved via a disentangled representation. For this, we explicitly construct an object-centric intermediate representation to characterize the states of an environment, which we refer to as `semantic tracklets.' We evaluate `semantic tracklets' on the visual multi-agent particle environment (VMPE) and on the challenging visual multi-agent GFootball environment. `Semantic tracklets' consistently outperform baselines on VMPE, and achieve a +2.4 higher score difference than baselines on GFootball. Notably, this method is the first to successfully learn a strategy for five players in the GFootball environment using only visual data.

==> fig_qual_results_single_football.tex <==
\begin{figure}[t]
\centering
\begin{tabular}{cc}
\includegraphics[width=0.45\linewidth, ]{fig/1Ma}&
\includegraphics[width=0.45\linewidth, ]{fig/5Ma}\\
\scriptsize(a) & \scriptsize(b)\\
\includegraphics[width=0.45\linewidth, ]{fig/1Mb}&
\includegraphics[width=0.45\linewidth, ]{fig/5Mb}\\
\scriptsize(d) & \scriptsize(e)\\
\end{tabular}
\caption{Qualitative results: semantic tracklets for controlling three agents. We visualize the trajectory of the ball in {\bf \color{yy} yellow}. The thickness of the line indicates the time direction, \ie, the thicker the more recent in time.
}
\label{fig:qual_result_single_football}
\end{figure}
